Convergence and Optimality of Policy Gradient Methods in Weakly Smooth Settings

Policy gradient methods have been frequently applied to problems in control and reinforcement learning with great success, yet existing convergence analysis still relies on non-intuitive, impractical and often opaque conditions. In particular, existing rates are achieved in limited settings, under strict regularity conditions. In this work, we establish explicit convergence rates of policy gradient methods, extending the convergence regime to weakly smooth policy classes with $L_2$ integrable gradient. We provide intuitive examples to illustrate the insight behind these new conditions. Notably, our analysis also shows that convergence rates are achievable for both the standard policy gradient and the natural policy gradient algorithms under these assumptions. Lastly we provide performance guarantees for the converged policies.

==> 5-analysis.tex <==
\section{Analysis}
\subsection{Convergence}
We provide a brief sketch of our proofs, including key lemmas. The full details are deferred to the appendix. Firstly, we show that under weak integrability assumptions, that limiting distributions exist for policies acting on the MDP. Subsequently we establish geometric ergodicity for near-linear MDPs under our assumptions:

\begin{lemma}
    (Ergodicity of near-Linear MDPs) Under assumptions \ref{as:smooth} and \ref{as:chain}, state-distributions on linear MDPs satisfy the following ergodicity property (up to polylogarithmic factors):
    \begin{equation}
        \hspace{-0.14in} \int f(s) \sq{\Prob^n_{\theta}(s'|s_0 = s) - \rho_*(s')} ds \leq C_{erg} f(s') \kappa^n,
    \end{equation}
    where $\Prob^k_{\theta}(x_1|x_2)$ represents the probability of $s_k = x_1$ if $s_0 = x_0$ and actions are selected through $\pi_{\theta}$ (i.e. the $k$-step transition kernel of the generated Markov Chain), and $\abs{f(s)} \leq \max(\sqrt{L}(s), L(s))$ is a Lyapunov function. $C_{erg} \geq 0, \kappa \in (0,1)$ are constants independent of $\theta, s$ and $\rho_*$ is the limiting distribution of the Markov Chain.
    \label{lem:erg}
\end{lemma}

\textbf{Remarks:} This results uses the notion of geometric ergodicity, which is weaker than the uniform ergodicity assumed in some prior work \cite{xu2020improving}. Nonetheless it is sufficient to show the correct smoothness bounds. It describes the convergence of policies (with respect to state space distributions) in exponential time, which is an important stabilizing result.

Subsequently, using perturbation results on Markov Chains, the following bound holds for the state transition kernels (again up to polylogarithmic factors):
\begin{equation}
        \norm{\Prob^n_{\theta} - \Prob^n_{{\theta+\eta}}} \leq C_{12} \norm{\Prob_\theta^1, \Prob_{\theta+\eta}^1},
\end{equation}
Then, using standard Markov chain analysis, we can use this result to show weak smoothness on the Q-function and induced visitation distributions, by using the weak smoothness of the policy itself.

Consequently, we can use this to bound the smoothness of the RL objective function (\ref{eq:obj}) through the following proposition:

\begin{prop}
    (Smoothness of MDPs) Under Assumptions \ref{as:smooth}, \ref{as:moment} and either \ref{as:chain} or assuming the result of Lemma \ref{lem:erg}, the objective function is (locally)-weakly smooth:
    \begin{equation}
        \norm{\nabla J(\theta) - \nabla J(\theta+\eta)} \leq \frac{C_{J}}{1-\gamma} \norm{\eta}^{\holder},
    \end{equation}
    for $\norm{\eta} \leq C_{\eta}$, with $C_{J}$ a problem dependent parameter, and $\holder = \min(\sqrt{\beta_1}, \beta_2)$ is the coefficient of weak smoothness. 
    \label{prop:smooth}
\end{prop}

\textbf{Remarks:} If assumption (\ref{as:moment}) is strengthened to $L_q$ integrability for $q \in [2, \infty]$ will lead to smoothly interpolated $\holder = \min(\beta_1^r, \beta_2)$ for $r \in [\frac{1}{2}, 1]$ via a Hölder inequality. In the limiting case, this is recovers the Lipschitz smoothness property that is relied upon in prior work.

Once smoothness is established, we apply analysis of the iterates based on stochastic approximation principles. We note that due to the weak smoothness, constant learning rates $h_t = c$ do not guarantee stepwise contraction of the iterates $J(\theta_t)$ with high probability (since the first order expansion and the remainder terms have differing orders in $\norm{\nabla J}$ when applying Taylor's theorem). Instead, our choice of $\theta$ guarantees that the first-order term dominates over the truncation error.

Secondly, our Assumption \ref{as:moment} is sufficient to bound the variance of the noise term. Thus, by appropriately shrinking the learning rate, we achieve our final convergence rate. The analysis for natural policy gradient does not significantly differ, only accounting for the scaling due to the matrix $\Exp \norm{K_t} = O(\psi_{\infty, 1})$.

\subsection{Optimality}
Optimality results for natural policy gradient can be obtained by bounding the KL divergences, whose difference can be written as:
\begin{align}
&D_{KL}(\theta_*, \theta_t) - D_{KL}(\theta_*, \theta_{t-1}) = \\
&\Exp_{s, a \sim d_{*}} \sq{\log \pi_{\theta_{t-1}}(a|s) - \log \pi_{\theta_t}(a|s)},
\end{align}
which can be controlled using our previously established bounds on the gradient as a function of $T$. The bound is dominated by the gap between our estimator $(K_t + \xi I)^{-1}$ from the true information matrix $K(\theta_t)^\dagger$; the analysis is complicated by $\norm{\nabla J(\theta)}$ being present in the learning rate, which leads to the additional terms present in our theorem compared to the smooth case.

For standard policy gradient, without additional assumptions it is not possible to estimate the optimality of our policy. Using a global convexity-like property such as Assumption \ref{as:smooth}, we can establish a form of gradient domination:

\begin{lemma}
        (Gradient Domination Lemma) Under assumptions, then for any policy $\pi_\theta$, the following global bound holds:
        \begin{equation}
            V_{\theta_1}(\rho) - V_{\theta_2}(\rho) \leq \frac{1}{(1-\disc)} D_\infty  \norm{\theta_1 - \theta_2}^p \norm{\nabla_\theta J(\pi_{\theta_2})},
        \end{equation}
        for any two policies $\pi_{\theta_1}, \pi_{\theta_2}$, any state distribution $\rho \in \Delta(\State)$, and $D_\infty = \norm{\frac{D d_{\theta_1,\rho}}{\rho}}_\infty$ measures the regularity of the initial distribution.   
\end{lemma}

Subsequently, we easily can find a global optimality result by bounding the difference $J_* - J(\theta_t)$, which is accelerated by increasing $p$. In particular, we find that $p=1$ yields an order of optimality which is not dependent on the smoothness parameter $\holder$.


